Secure Parsing and Serializing with Separation Logic Applied to CBOR, CDDL, and COSE

Incorrect handling of security-critical data formats, particularly in low-level languages, are the root cause of many security vulnerabilities. Provably correct parsing and serialization tools that target languages like C can help. Towards this end, we present PulseParse, a library of verified parser and serializer combinators for non-malleable binary formats. Specifications and proofs in PulseParse are in separation logic, offering a more abstract and compositional interface, with full support for data validation, parsing, and serialization. PulseParse also supports a class of recursive formats -- with a focus on security and handling adversarial inputs, we show how to parse such formats with only a constant amount of stack space. We use PulseParse at scale by providing the first formalization of CBOR, a recursive, binary data format standard, with growing adoption in various industrial standards. We prove that the deterministic fragment of CBOR is non-malleable and provide EverCBOR, a verified library in both C and Rust to validate, parse, and serialize CBOR objects implemented using PulseParse. Next, we provide the first formalization of CDDL, a schema definition language for CBOR. We identify well-formedness conditions on CDDL definitions that ensure that they yield unambiguous, non-malleable formats, and implement EverCDDL, a tool that checks that a CDDL definition is well-formed, and then produces verified parsers and serializers for it. To evaluate our work, we use EverCDDL to generate verified parsers and serializers for various security-critical applications. Notably, we build a formally verified implementation of COSE signing, a standard for cryptographically signed objects. We also use our toolchain to generate verified code for other standards specified in CDDL, including DICE Protection Environment, a secure boot protocol standard.

==> lstfstar.tex <==
\makeatletter
\lstdefinelanguage{fstar}{%
  basicstyle=\small,
  morekeywords=[1]{type,and,val,fun,let,in,try,if,then,else,match,with,open,as,module,rec,begin,end,assume,private,when,forall,assert,by_tactic,logic,pattern,effect,requires,ensures,decreases,modifies, abstract,total, reifiable, reflectable, new, new_effect, effect_actions, noeq, sub_effect, by,splice,class},
  morekeywords=[2]{WP, Post, Pre, Pure , PURE, DIV, STATE, EXN, ALL, TotST, M, GHOST, Ghost, GTot, Lemma, Tot, Div, DIV, Memo, READER, STATE_m, Effect, STEXN, RANDOM, ST, St, MST, S_MST, MSTExn, TAC, Tac, TacH, Dv},
  morekeywords=[3]{},
  morekeywords=[4]{},
  morestring=[b]",
  sensitive=true,%
  numbersep=4pt,
  columns=[l]fullflexible,
  texcl=true,
  mathescape=true,
  identifierstyle={\sffamily},
  keywordstyle=[1]{\sffamily\bfseries\maybecolor{dkblue}},
  keywordstyle=[2]{\sffamily\bfseries\maybecolor{dkblue}},
  keywordstyle=[3]{\itshape\maybecolor{dkred}},
  keywordstyle=[4]{\rmfamily\itshape},
  rangeprefix=(*---\ ,
  includerangemarker=false,
  stringstyle=\ttfamily,
  showspaces=false,
  morecomment=[n]{(*}{*)},
  commentstyle={\itshape\maybecolor{dkred}},
  literate={->}{$\rightarrow$}{1}
           {_'a}{${}_\alpha$}{1}
           {_\{'a+1\}}{${}_{\alpha+1}$}{2}
           {_\{i\}}{${}_{\mathsf{i}}$}{2}
           {_\{i+1\}}{${}_{\mathsf{i}+1}$}{2}
           {__}{\_}{1}
           {exists}{$\exists$}{1}
           {forall}{$\forall$}{1}
           {fun\ }{$\lambda$ }{2}
           {func}{func}{1}
           {~}{$\neg$}{1}           
           {~>}{$\leadsto$}{1}
           {`}{\`{}}{1}
           {'a}{$\alpha$}{1}
           {'b}{$\beta$}{1}
           {'c}{$\gamma$}{1}
           {phi}{$\phi$}{1}
           {tau}{$\tau$}{1}
           {tauto}{tauto}{6}
           {psi}{$\psi$}{1}
           {xi}{$\xi$}{1}
           {VC_e}{VC$_e$}{1}
           {Gamma}{$\Gamma$}{1}
           {theta}{$\theta$}{1}
           {_0}{$_0$}{1}
           {_1}{$_1$}{1}
           {_2}{$_2$}{1}
           {_3}{$_3$}{1}
           {_4}{$_4$}{1}
           {STATE0}{$\mathsf{ST}^\prime$}{1}
           {/\\}{$\wedge$}{1}
           {\\/}{$\vee$}{1}
           {>=}{$\geq$}{2}
           {<=}{$\leq$}{2}
           {<==>}{$\Longleftrightarrow$}{3}
           {==>}{$\Longrightarrow$}{3}
           {|->}{$\mapsto$}{3}
           {|>}{$\mapsto$}{2}
           {-~-}{$\bowtie$}{2}
           {.+}{$\odot$}{1}
           {`compose`}{$\circ$}{1}
           {later_credit\ }{\textsterling}{1}
           {later\ }{$\rhd$}{1}
           {`equiv`}{$\equiv$}{1}
           {pulseup}{$\uparrow$}{1}
           {pulsedown}{$\downarrow$}{1}
     {<>}{$\neq$}{1}
     {<*>}{$\bullet \ $}{3}
     {--}{-}{1}   %
     {<<}{$\prec\ $}{1}
           ,
  breaklines=false}
\makeatother



==> lstpulse.tex <==
\lstdefinelanguage{pulse}{%
  basicstyle=\small,
  morekeywords=[1]{type,val,if,then,else,match,let,fold,unfold,rewrite,drop,with_invariants,each,as},
  morekeywords=[2]{requires,returns,ensures,ghost,fn,atomic,opens,rec,function},
  morekeywords=[3]{},
  morekeywords=[4]{},
  morestring=[b]",
  sensitive=true,%
  numbersep=4pt,
  columns=[l]fullflexible,
  texcl=true,
  mathescape=true,
  identifierstyle={\sffamily},
  keywordstyle=[1]{\sffamily\bfseries\maybecolor{dkblue}},
  keywordstyle=[2]{\sffamily\bfseries\maybecolor{dkblue}},
  keywordstyle=[3]{\itshape\maybecolor{dkred}},
  keywordstyle=[4]{\rmfamily\itshape},
  rangeprefix=(*---\ ,
  includerangemarker=false,
  stringstyle=\ttfamily,
  showspaces=false,
  morecomment=[n]{(*}{*)},
  commentstyle={\itshape\maybecolor{dkred}},
  literate={->}{$\rightarrow$}{1}
           {**}{$**$}{1}
           {__}{\_}{1}
           {exists}{$\exists$}{1}
           {forall}{$\forall$}{1}
           {fun\ }{$\lambda$ }{2}
           {~}{$\neg$}{1}           
           {'a}{$\alpha$}{1}
           {'b}{$\beta$}{1}
           {'c}{$\gamma$}{1}
           {'t}{$\tau$}{1}
           {'p}{$\phi$}{1}
           {'q}{$\psi$}{1}
           {'v}{$\nu$}{1}                                 
           {_0}{$_0$}{1}
           {_1}{$_1$}{1}
           {_2}{$_2$}{1}
           {_3}{$_3$}{1}
           {_4}{$_4$}{1}
           {/\\}{$\wedge$}{1}
           {\\/}{$\vee$}{1}
           {>=}{$\geq$}{2}
           {<=}{$\leq$}{2}
           {<==>}{$\Longleftrightarrow$}{3}
           {==>}{$\Longrightarrow$}{3}
           {later_credit\ }{\textsterling}{1}
           {later\ }{$\rhd$}{1}
           {`equiv`}{$\equiv$}{1}
           {<>}{$\neq$}{1}
           {--}{-}{1}   %
           {<<}{$\prec\ $}{1}
           ,
  breaklines=false}
\makeatother

